Quaternion Equivariant Capsule Networks for 3D Point Clouds

We present a 3D capsule module for processing point clouds that is equivariant to 3D rotations and translations, as well as invariant to permutations of the input points. The operator receives a sparse set of local reference frames, computed from an input point cloud and establishes end-to-end transformation equivariance through a novel dynamic routing procedure on quaternions. Further, we theoretically connect dynamic routing between capsules to the well-known Weiszfeld algorithm, a scheme for solving \emph{iterative re-weighted least squares} (IRLS) problems with provable convergence properties. It is shown that such group dynamic routing can be interpreted as robust IRLS rotation averaging on capsule votes, where information is routed based on the final inlier scores. Based on our operator, we build a capsule network that disentangles geometry from pose, paving the way for more informative descriptors and a structured latent space. Our architecture allows joint object classification and orientation estimation without explicit supervision of rotations. We validate our algorithm empirically on common benchmark datasets.

==> RelatedWork.tex <==
\section{Related Work}
\label{sec:related}
This section briefly review the existing work that is most related to our approach. A more exhaustive survey of existing research, tackling the fields of point cloud processing, equivariance in neural networks and capsule networks, is presented in~\cref{sec:extendedrelated}.

Capsule networks have been introduced by \cite{hinton2011transforming} and brought to main-stream interest by \cite{sabour2017dynamic}, who proposed the \textit{dynamic routing by agreement} procedure.  Since then, routing by agreement has been connected to several well-known concepts, e.g. the EM algorithm \cite{sabour2018matrix}, clustering with KL divergence regularization \cite{wang2018an} and equivariance \citep{lenssen2018group}. Our work connects to this line of work by extending the concept to the 3D rotation group $SO(3)$.

A successful approach to achieve theoretically well-founded equivariance in deep neural networks consists of \textit{group equivariant convolutions} \cite{cohen2016group, cohen2016steerable}, often combined with harmonic basis filters \citep{Weiler_2018_CVPR, Worrall_2017_CVPR}, which are parameterized to continuously cover the group. Several extensions to 3D exist for voxel  \citep{Worrall_2018_ECCV} or spherical representations \citep{cohen2018spherical, esteves2018learning, weiler20183d}. The methods consider input data lying on the unit sphere and are not directly applicable to point clouds. These approaches have in common that they require dense group discretization in feature space, which leads to suffering from high time complexity and a large memory footprint for higher-dimensional groups like $SO(3)$. Also, they do not allow direct read-out of group elements. In contrast, our approach achieves equivariance on a sparse set of group elements, and output elements contain interpretable information about object pose.

Closely related are \textit{Tensor Field Networks} (TFN)~\citep{thomas2018tensor}, which come with localized filters that are equivariant to rotations, translations and permutations. Based on a geometric algebra framework the authors achieve equivariance on a field of orientation tensors.




\insertimageStar{1}{shpaeAlign_cropped.pdf}{Shape alignment on the \textbf{monitor} (left) and \textbf{toilet} (right) objects via our siamese equivariant capsule architecture. The shapes are assigned to the the maximally activated class. The corresponding pose capsule provides the rotation estimate.}{fig:shapeAlign}{t!}



